Combinatorial specification of permutation classes

This article presents a methodology that automatically derives a combinatorial specification for the permutation class C = Av(B), given its basis B of excluded patterns and the set of simple permutations in C, when these sets are both finite. This is achieved considering both pattern avoidance and pattern containment constraints in permutations.The obtained specification yields a system of equations satisfied by the generating function of C, this system being always positiveand algebraic. It also yields a uniform random sampler of permutations in C. The method presentedis fully algorithmic.

==> header.tex <==
\pagestart{1}

\pageend{12}
\authorhead{ F. Bassino  and M. Bouvel  and A. Pierrot  and C. Pivoteau  and D. Rossin}
\titlehead{Combinatorial specification of permutation classes}
\titlelong{Combinatorial specification of permutation classes}
\keywords{permutation classes, excluded patterns, substitution decomposition, simple permutations, generating functions, combinatorial specification, random generation}


